Many regular triangulations and many polytopes

We show that for fixed $d>3$ and $n$ growing to infinity there are at least $(n!)^{d-2 \pm o(1)}$ different labeled combinatorial types of $d$-polytopes with $n$ vertices. This is about the square of the previous best lower bounds. As an intermediate step, we show that certain neighborly polytopes (such as particular realizations of cyclic polytopes) have at least $(n!)^{ \lfloor(d-1)/2\rfloor \pm o(1)}$ regular triangulations.

==> Figures/hexagon1.tex <==
%%%%%%%%%%%%%%%%%%%%%%% this part (as well as the \end{document}) has to be commented when we compile the main file, but it can be uncommented if we want to see quicly our modifications)

%\documentclass[tikz,border=10pt]{standalone}
%\usepackage{bm}%allows for bold math symbols with \bm
%\usetikzlibrary{decorations.pathreplacing,decorations.markings,arrows,patterns}
%
%%\usepackage{color} %Joseph Doolittle's colors (adapted to color-blind people)
%%    \definecolor{orange}{rgb}{0.898, 0.621, 0.0}
%%    \definecolor{skyblue}{rgb}{0.336, 0.703, 0.910}
%%    \definecolor{bluishgreen}{rgb}{0, 0.617, 0.449}
%%    \definecolor{yellow}{rgb}{0.937, 0.890, 0.258}
%%    \definecolor{blue}{rgb}{0, 0.445, 0.695}
%%    \definecolor{red}{rgb}{0.832, 0.367, 0}
%%    \definecolor{purple}{rgb}{0.797, 0.473, 0.652}
%
%\begin{document}

%%%%%%%%%%%%%%%%%%%%%%%%%



% Macro for drawing a hexagon   
\def\hexa{\draw(p) -- (p1) -- (p2) -- (p3) -- (p5) -- (p4) -- cycle;}


\begin{tikzpicture}
    % Define the hexagon coordinates
    \coordinate (p) at (1.1,1.11);
    \coordinate (p1) at (0.3,1.88);
    \coordinate (p2) at (-0.76,1.54);
    \coordinate (p3) at (-0.76,0.69);
    \coordinate (p5) at (-0.10,0.16);
    \coordinate (p4) at (0.73,0.35);
    
    % Define the coordinates of the L_t figures
    \coordinate (q1) at (0, 1.8);
    \coordinate (q2) at (0, 1.2);
    \coordinate (q3) at (0, 0.6);
    \coordinate (q5) at (0, 0);
  
\matrix[column sep=0.8cm,row sep=0.5cm]
{
	\draw (q1)+(0,0.5) node[above]{$T$};
	\draw(p) -- (p1) -- (p2) -- (p3) -- (p5) -- (p4) -- cycle;
	\fill[BlueViolet!30] (p) -- (p1) -- (p2) -- (p3) -- (p4) -- cycle;
	   \draw (p) node[right]{$p$};
    \draw (p1) node[above]{$1$};
    \draw (p1) node[BlueViolet]{$\bullet$};
    \draw (p2) node[left]{$2$};
    \draw (p2) node[BlueViolet]{$\bullet$};
    \draw (p3) node[left]{$3$};
    \draw (p3) node[BlueViolet]{$\bullet$};
    \draw (p5) node[below]{$4$};
    \draw (p4) node [below]{$5$};
    \draw (p4) node[BlueViolet]{$\bullet$};
	\draw[thick, BlueViolet] (p1) -- (p2) -- (p3) -- (p4);
    \draw \foreach \x/\y in {p/p2, p/p3, p3/p4} {(\x)--(\y)};
	&
    \draw (q1)+(0,0.5) node[above]{$T/p$};
	\draw [BlueViolet] \foreach \x in {1,2,3,5} {(q\x) node{$\bullet$}};
	\draw \foreach \x in {1,2,3,5} {(q\x) node[left]{$\x$}};
	\draw [thick,BlueViolet] \foreach \x in {1,2,3,5} \foreach \y in {1,2,3,5} {(q\x) -- (q\y)};\\
};
    
    
\end{tikzpicture}



%%%%%%%%%%%% to comment when we compile the main file
%\end{document}


==> Figures/proof_inductionstep.tex <==
%%%%%%%%%%%%%%%%%%%%%%% this part (as well as the \end{document}) has to be commented when we compile the main file, but it can be uncommented if we want to see quicly our modifications)
%
%\documentclass[tikz,border=10pt]{standalone}
%\usepackage{bm}%allows for bold math symbols with \bm
%\usetikzlibrary{decorations.pathreplacing,decorations.markings,arrows,patterns}
%
%%\usepackage{color} %Joseph Doolittle's colors (adapted to color-blind people)
%%    \definecolor{orange}{rgb}{0.898, 0.621, 0.0}
%%    \definecolor{skyblue}{rgb}{0.336, 0.703, 0.910}
%%    \definecolor{bluishgreen}{rgb}{0, 0.617, 0.449}
%%    \definecolor{yellow}{rgb}{0.937, 0.890, 0.258}
%%    \definecolor{blue}{rgb}{0, 0.445, 0.695}
%%    \definecolor{red}{rgb}{0.832, 0.367, 0}
%%    \definecolor{purple}{rgb}{0.797, 0.473, 0.652}
%
%\begin{document}

%%%%%%%%%%%%%%%%%%%%%%%%%



% Macro for drawing a heptagon   
\def\hepta{\draw(p) -- (p') -- (p1) -- (p2) -- (p3) -- (p5) -- (p4) -- cycle;}
\def\hexa{\draw(p) -- (p1) -- (p2) -- (p3) -- (p5) -- (p4) -- cycle;}


% Macro for drawing polygon diagonals. 
% Example \slice{A/C,C/E,E/G,C/G}

\newcommand{\triang}[3]{%draw the diagonals of the polygon, first set = diagonals adjacent to p minus the first one; second set = diagonals adjacent to p' minus the last one ; third set = {vertex adjacent to p and p'}
    \fill[color=RedOrange!30] (p) -- (p#3) -- (p') -- cycle;
    \draw (p) -- (p');
    \draw \foreach \x in {#1} {(p)--(p\x)};
    \draw \foreach \y in {#2} {(p')--(p\y)};
    \draw [thick, RedOrange] (p) -- (p#3);
    \draw [thick, RedOrange] (p#3) -- (p');
    \draw (p3) -- (p5) -- (p4) ;
    \draw [thick, RedOrange] (p#3) node{$\bullet$};
    \draw [BlueViolet] \foreach \x in {#1} {(p\x) node{$\bullet$}};
    \draw [PineGreen] \foreach \x in {#2} {(p\x) node{$\bullet$}};
    \draw (p) node[right]{$p$};
    \draw (p') node[right]{$p'$};
    \draw (p1) node[above]{$1$};
    \draw (p2) node[left]{$2$};
    \draw (p3) node[left]{$3$};
    \draw (p5) node[below]{$4$};
    \draw (p4) node [below]{$5$};

}

\newcommand{\Lt}[3]{%draw the figures $L_t$ and $L_t'$, the first set corresponds to the indices of vertices in L_t, the second one to indices of vertices in L_t'
	\draw (q1)+(0,0.2) node[above]{$L_{t_{#3}}$};
	\draw [BlueViolet] \foreach \x in {#1} {(q\x) node{$\bullet$}};
	\draw \foreach \x in {#1} {(q\x) node[left]{$\x$}};
	\draw [thick, BlueViolet] \foreach \x in {#1} \foreach \y in {#1} {(q\x) -- (q\y)};
	
	\draw (q1')+(0,0.2) node[above]{$L_{t_{#3}}'$};
	\draw [PineGreen] \foreach \x in {#2} {(q\x ') node{$\bullet$}};
	\draw \foreach \x in {#2} {(q\x ') node[left]{$\x$}};
	\draw [thick, PineGreen] \foreach \x in {#2} \foreach \y in {#2} {(q\x ') -- (q\y ')};
}

\begin{tikzpicture}
    % Define the heptagon coordinates
    \coordinate (p) at (1.1,1.11);
    \coordinate (p') at (1, 1.5);
    \coordinate (p1) at (0.3,1.88);
    \coordinate (p2) at (-0.76,1.54);
    \coordinate (p3) at (-0.76,0.69);
    \coordinate (p5) at (-0.10,0.16);
    \coordinate (p4) at (0.73,0.35);
    
    % Define the coordinates of the L_t figures
    \coordinate (q1) at (0, 1.5);
    \coordinate (q2) at (0, 1);
    \coordinate (q3) at (0, 0.5);
    \coordinate (q5) at (0, 0);
    \coordinate (q1') at (1, 1.5);
    \coordinate (q2') at (1, 1);
    \coordinate (q3') at (1, 0.5);
    \coordinate (q5') at (1, 0);
  
\matrix[column sep=0.5cm,row sep=0.5cm]
{   
	\draw (q1)+(0,0.7) node[above]{$T$};

	\fill[BlueViolet!30] (p) -- (p1) -- (p2) -- (p3) -- (p4) -- cycle;
\draw(p) -- (p1) -- (p2) -- (p3) -- (p5) -- (p4) -- cycle;
	\draw[thick, BlueViolet] (p1) -- (p2) -- (p3) -- (p4);
    \draw \foreach \x/\y in {p/p2, p/p3} {(\x)--(\y)};
	   \draw (p) node[right]{$p$};
    \draw (p1) node[above]{$1$};
    \draw (p1) node[BlueViolet]{$\bullet$};
    \draw (p2) node[left]{$2$};
    \draw (p2) node[BlueViolet]{$\bullet$};
    \draw (p3) node[left]{$3$};
    \draw (p3) node[BlueViolet]{$\bullet$};
    \draw (p5) node[below]{$4$};
    \draw (p4) node [below]{$5$};
    \draw (p4) node[BlueViolet]{$\bullet$};
	&&
	
	\draw (q1)+(0,0.7) node[above]{$T_{t_1}$};
    \fill[color=BlueViolet!30] (p) -- (p1) -- (p2) -- (p3) -- (p4) -- cycle;
    \draw [thick, BlueViolet] (p1) -- (p2) -- (p3) -- (p4);
    \triang{2, 3, 4}{}{1};&

    \draw (q1)+(0,0.7) node[above]{$T_{t_2}$};
    \fill[color=BlueViolet!30] (p) -- (p2) -- (p3) -- (p4) -- cycle;
    \draw [thick, BlueViolet] (p2) -- (p3) -- (p4);
    \fill[color=PineGreen!30] (p') -- (p1) -- (p2) -- cycle;
    \draw [thick, PineGreen] (p1) -- (p2);
    \triang{3, 4}{1}{2}; &

    \draw (q1)+(0,0.7) node[above]{$T_{t_3}$};
    \fill[color=BlueViolet!30] (p) -- (p3) -- (p4) -- cycle;
    \draw [thick, BlueViolet] (p3) -- (p4);
    \fill[color=PineGreen!30] (p') -- (p1) -- (p2) -- (p3) -- cycle;
    \draw [thick, PineGreen] (p1) -- (p2) -- (p3);
    \triang{4}{1, 2}{3}; &
    
    \draw (q1)+(0,0.7) node[above]{$T_{t_4}$};
    \fill[color=PineGreen!30] (p') -- (p1) -- (p2) -- (p3) -- (p4)-- cycle;
    \draw [thick, PineGreen] (p1) -- (p2) -- (p3) -- (p4);
    \triang{}{1, 2, 3}{4};\\   
    \draw (q1)+(0,0.2) node[above]{$T/p$};
	\draw [BlueViolet] \foreach \x in {1,2,3,5} {(q\x) node{$\bullet$}};
	\draw \foreach \x in {1,2,3,5} {(q\x) node[left]{$\x$}};
	\draw [thick,BlueViolet] \foreach \x in {1,2,3,5} \foreach \y in {1,2,3,5} {(q\x) -- (q\y)};&&
    \Lt{1, 2, 3, 5}{1}{1}; &
    \Lt{2, 3, 5}{1, 2}{2}; &
    \Lt{3, 5}{1, 2, 3}{3}; &
    \Lt{5}{1, 2, 3, 5}{4};\\
};
    
    
\end{tikzpicture}

%%%%%%%%%%%% to comment when we compile the main file
%\end{document}

